Hadronic B Decays to Charmless Final States and to J/psi K*

Preliminary results from the BABAR experiment on charmless B decays to charged pions or kaons, and the measurement of the B -> J/psi K* decay amplitudes are presented. The data sample, collected at the asymmetric-energy B-factory PEP-II at SLAC, comprises a total number of 22.7 million Y(4S) decays, corresponding to an integrated on-resonance luminosity of approximately 21 fb-1. We measure the following CP-averaged branching fractions: BR(B -> pi+pi-) = (4.1 +- 1.0(stat) +- 0.7(sys))xE-6 BR(B -> K+pi-) = (16.7 +- 1.6(stat) +1.2-1.7(sys))xE-6 and an upper limit of BR(B -> K+K-) < 2.5xE-6, at 90% confidence limit. The measurement of the J/psi K* decay amplitudes results in R_\perp = 0.160 +- 0.032(stat) +- 0.036(sys), and reveals a dominant longitudinal component. The phase of the longitudinal amplitude shows evidence for non-vanishing final state interaction.

==> pubboard/babarsym.tex <==
%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised    12/7/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised    7/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised    7/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised    7/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised    7/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised    7/01/00 D. MacFarlane
%%%%%   Revised    6/21/00 D. Hitlin
%%%%%   Original   6/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
% \def\babar{ BABAR}
\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
%\usepackage{relsize}
%\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
%    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {{e}\xspace}
\def\en         {{e^-}\xspace}      % electron negative (\em is taken)
\def\ep         {{e^+}\xspace}
\def\epm        {{e^\pm}\xspace} 
\def\epem       {{e^+e^-}\xspace}
\def\ee         {{e^-e^-}\xspace}
\def\mmu        {{\mu}\xspace}
\def\mup        {{\mu^+}\xspace}
\def\mun        {{\mu^-}\xspace}    % muon negative (\mum is taken)
\def\mumu       {{\mu^+\mu^-}\xspace}
\def\mtau       {{\tau}\xspace}
\def\taup       {{\tau^+}\xspace}
\def\taum       {{\tau^-}\xspace}
\def\tautau     {{\tau^+\tau^-}\xspace}
\def\ellm       {{\ell^-}\xspace}
\def\ellp       {{\ell^+}\xspace}
\def\ellell     {{\ell^+ \ell^-}\xspace}
\def\nub        {{\overline{\nu}}\xspace}
\def\nunub      {{\nu{\overline{\nu}}}\xspace}
\def\nub        {{\overline{\nu}}\xspace}
\def\nunub      {{\nu{\overline{\nu}}}\xspace}
\def\nue        {{\nu_e}\xspace}
\def\nueb       {{\nub_e}\xspace}
\def\nuenueb    {{\nue\nueb}\xspace}
\def\num        {{\nu_\mu}\xspace}
\def\numb       {{\nub_\mu}\xspace}
\def\numnumb    {{\num\numb}\xspace}
\def\nut        {{\nu_\tau}\xspace}
\def\nutb       {{\nub_\tau}\xspace}
\def\nutnutb    {{\nut\nutb}\xspace}
\def\nul        {{\nu_\ell}\xspace}
\def\nulb       {{\nub_\ell}\xspace}
\def\nulnulb    {{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {{\gamma}\xspace}
\def\gaga  {{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{{\gamma\gamma^*}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  LEPTONS, PHOTONS and other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ega   {{e\gamma}\xspace}
\def\game  {{\gamma e^-}\xspace}
\def\epemg  {{e^+e^-\gamma}\xspace}
\def\H  {{H^0}\xspace}
\def\Hp     {{H^+}\xspace}
\def\Hm     {{H^-}\xspace}
\def\Hpm    {{H^\pm}\xspace}
\def\W      {{W}\xspace}
\def\Wp     {{W^+}\xspace}
\def\Wm     {{W^-}\xspace}
\def\Wpm    {{W^\pm}\xspace}
\def\Z      {{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q   {{q}\xspace}
\def\qbar  {{\overline q}\xspace}
\def\qqbar {{q\overline q}\xspace}
\def\u  {{u}\xspace}
\def\ubar  {{\overline u}\xspace}
\def\uubar {{u\overline u}\xspace}
\def\d  {{d}\xspace}
\def\dbar  {{\overline d}\xspace}
\def\ddbar {{d\overline d}\xspace}
\def\s  {{s}\xspace}
\def\sbar  {{\overline s}\xspace}
\def\ssbar {{s\overline s}\xspace}
\def\c  {{c}\xspace}
\def\cbar  {{\overline c}\xspace}
\def\ccbar {{c\overline c}\xspace}
\def\b  {{b}\xspace}
\def\bbar  {{\overline b}\xspace}
\def\bbbar {{b\overline b}\xspace}
\def\t  {{t}\xspace}
\def\tbar  {{\overline t}\xspace}
\def\tbar  {{\overline t}\xspace}
\def\ttbar {{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   HADRONS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {{\pi^0}\xspace}
\def\pizs  {{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {{\pi^0\pi^0}\xspace}
\def\pip   {{\pi^+}\xspace}
\def\pim   {{\pi^-}\xspace}
\def\pipi  {{\pi^+\pi^-}\xspace}
\def\pipm   {{\pi^\pm}\xspace}
\def\pimp   {{\pi^\mp}\xspace}
\def\kaon  {{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {{\Kbar}\xspace}
\def\Kpm   {{K^\pm}\xspace}
\def\Kmp   {{K^\mp}\xspace}
\def\Kp    {{K^+}\xspace}
\def\Km    {{K^-}\xspace}
\def\KS    {{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {{K^{*0}}\xspace}
\def\Kstarzb  {{\Kbar^{*0}}\xspace}
\def\Kstar   {{K^*}\xspace}
\def\Kstarb  {{\Kbar^*}\xspace}
\def\Kstarp   {{K^{*+}}\xspace}
\def\Kstarm   {{K^{*-}}\xspace}
\def\Kstarpm   {{K^{*\pm}}\xspace}
\def\Kstarmp   {{K^{*\mp}}\xspace}
\def\Kz   {{K^0}\xspace}
\def\Kzb   {{\Kbar^0}\xspace}
\def\KzKzb {{K^0 \kern -0.16em \Kzb}\xspace}
\def\Dz    {{D^0}\xspace}
%%% do NOT use ensuremath here
\def\Dbar  {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db    {{\Dbar}\xspace}
\def\Dzb   {{\Dbar^0}\xspace}
\def\DzDzb {{D^0 {\kern -0.16em \Dzb}}\xspace}
\def\Dstar   {{D^*}\xspace}
\def\Dstarb   {{\Dbar^*}\xspace}
\def\Dstarz  {{D^{*0}}\xspace}
\def\Dstarzb  {{\Dbar^{*0}}\xspace}
\def\Ds    {{D^+_s}\xspace}
\def\Dsb   {{\Dbar^+_s}\xspace}
\def\Dss   {{D^*_s}\xspace}
\def\Bz    {{B^0}\xspace}
\def\B     {{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar  {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb    {{\Bbar}\xspace}
\def\Bzb   {{\Bbar^0}\xspace}
\def\Bu    {{B^+}\xspace}
\def\Bub   {{B^-}\xspace}
\def\Bpm   {{B^\pm}\xspace}
\def\Bs    {{B_s}\xspace}
\def\Bsb   {{\Bbar_s}\xspace}
\def\BB    {{B\Bbar}\xspace} 
\def\BzBzb {{B^0 {\kern -0.16em \Bzb}}\xspace}

\def\jpsi  {{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos {{\psi{(2S)}}\xspace}
\def\psiprpr {{\psi(3770)}\xspace}
\def\etac    {{\eta_c}\xspace}
\def\chiczero {{\chi_{c0}}\xspace}
\def\chicone {{\chi_{c1}}\xspace}
\def\chictwo {{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\X {{X}}

\def\proton     {{p}\xspace}
\def\antiproton {{\overline p}\xspace}
\def\neutron    {{n}\xspace}
\def\antineutron  {{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A
%%% do NOT use ensuremath here
\def\Deltabar   {\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar {\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  BRANCHING RATIOS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR{{{\cal B}}}
\def\BRtauptoe  {{\BR(\taup \to \ep)}}
\def\BRtaumtoe  {{\BR(\taum \to \en)}}
\def\BRtauptomu {{\BR(\taup \to \mup)}}
\def\BRtaumtomu {{\BR(\taum \to \mun)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  REACTIONS    %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb {{\Upsilon{\rm( 4S)}\to B\Bbar}} 
\def\upsbzbz {{\Upsilon{\rm( 4S)}\to\BzBzb}} 
\def\upsbpbm {{\Upsilon{\rm( 4S)}\to\Bu\Bub}} 
\def\bpsiks{{B^0 \to \jpsi \KS}}
\def\bpsikst{{B^0 \to \jpsi \Kstar}}
\def\bpsikl{{B^0 \to \jpsi \KL}}
\def\bpsikzeropi{{B^0 \to \jpsi (K^{*0} \to \KL\pi^0)}}
\def\bpsikpluspi{{B^+ \to \jpsi K^{*+},\ K^{*+} \to \KL\pi^+}}
\def\bpsikpluspi{{
{\Bz}/B^0 \to \jpsi ( \to \mu^+ \mu^-) K^{\pm} \pi^{\mp} }}
\def\bupsik{{B^{\pm} \to \jpsi ( \to \mu^+ \mu^-) K^{\pm} }}
\def\bpsiX{{B^0 \to \jpsi X}}
\def\upspsikl{{\FourS\to (\bpsikl) (\bzb \to X)}}
\def\Bzbtomu    {{\Bzb \to \mu {\rm X}}}
\def\Bzbtox     {{\Bzb \to {\rm X}}}
\def\Bztopipi   {{B^0 \to \pipi}}
\def\Bztokpi    {{B^0 \to K^{+}\pi^{-}}}
\def\Bztokk     {{B^0 \to K^+K^-}}
\def\Bztorhopi  {{B^0 \to \rho^+\pi^-}}
\def\Bztorhorho {{B^0 \to \rho\rho}}
\def\Bztokrho   {{B^0 \to K\rho}}
\def\Bztokstpi  {{B^0 \to \Kstar\pi}}
\def\Bztoapi    {{B^0 \to a_1\pi}}
\def\Bztodd     {{B^0 \to D^+D^-}}
\def\Bztodstd   {{B^0 \to D^{*+}D^-}}
\def\Bztodstdst {{B^0 \to D^{*+}D^{*-}}}
\def\BtoDK      {{B \to DK}}
\def\Btodstlnu  {{B \to D^*l\nu}}
\def\Btodstdlnu {{B \to D^*(D)l\nu}}
\def\Btorholnu  {{B \to \rho l\nu}}
\def\Btopilnu   {{B \to \pi l\nu}}
\def\Btoetah    {{B \to \eta h}}
\def\Btoetaph   {{B \to \eta ' h}}
\def\tauptoe    {{\taup \to \ep \nu \overline \nu}}
\def\taumtoe    {{\taum \to \en \nu \overline \nu}}
\def\tauptomu   {{\taup \to \mup \nu \overline \nu}}
\def\taumtomu    {{\taum \to \mun \nu \overline \nu}}
\def\Btoetaph   {{B \to \eta ' h}}
\def\tauptopi   {{\taup \to \pip \overline \nu}}
\def\taumtopi   {{\taum \to \pim \nu}}
\def\ggtopi     {{\gaga \to \pipi}}
\def\ggtopiz    {{\gaga \to \ppz}}
\def\ggstox     {{\ggstar \to \X(1420) \to \kaon \kaon \pi}}
\def\ggstoeta   {{\ggstar \to \eta(550) \to \pipi \piz}}
\def\btosgam   {{b \to s \gamma}}
\def\btodgam   {{b \to d \gamma}}
\def\btosll    {{b \to s l^+l^-}}
\def\btosnunu   {{b \to s \nu\nub}}
\def\btosgaga   {{b \to s \gaga}}
\def\btosglue   {{b \to s g}}


% Kinematics

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}


% Geometry
\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos \theta$}\xspace}

% UNITS
%
\newcommand{\tev}{{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {{\rm \,e\kern -0.08em V}}
%\def\kev  {{\rm \,ke\kern -0.08em V}} 
%\def\mev  {{\rm \,Me\kern -0.08em V}} 
%\def\gev  {{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {{\rm \,Te\kern -0.08em V}}
%\def\mevc {{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{{{\rm \,Me\kern -0.08em V\!/}c^2}} 
\def\syin {{^{\prime\prime}}\xspace}
\def\inch   {{\rm \,in}\xspace} % \in is taken
\def\ft   {{\rm \,ft}\xspace}
\def\km   {{\rm \,km}\xspace}
\def\m    {{\rm \,m}\xspace}
\def\cm   {{\rm \,cm}\xspace}
\def\cma  {{{\rm \,cm}^2}\xspace}
\def\mm   {{\rm \,mm}\xspace}
\def\mma  {{{\rm \,mm}^2}\xspace}
%\def\mum  {{\rm \,\mum}\xspace}
\def\mum  {{\,\mu\rm m}\xspace}%% mu meter 
%\def\muma {{\rm \,\mum}^2\xspace}
\def\muma       {{\,\mu\rm m^2}\xspace}
\def\nm   {{\rm \,nm}\xspace}
\def\fm   {{\rm \,fm}\xspace}
%
\def\barn{{\rm \,b}\xspace}
\def\barnhyph{{\rm -b}\xspace}
\def\mbarn{{\rm \,mb}\xspace}
\def\mbarnhyph{{\rm -mb}\xspace}
\def\pb {{\rm \,pb}\xspace}
\def\invpb {{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {{\mbox{\,fb}}\xspace}
\def\invfb   {{\mbox{\,fb}^{-1}}\xspace}
%
\def\mus  {{\rm \,\mus}\xspace}
\def\ns   {{\rm \,ns}\xspace}
\def\ps   {{\rm \,ps}\xspace}
\def\fs   {{\rm \,fs}\xspace}
\def\gm   {{\rm \,g}\xspace}
%
\def\Xrad {{X_0}\xspace}
\def\NIL{{\lambda_{int}}\xspace}
\let\dgr\degrees

%
% Lengths / Areas
%
%\def\m          {{\rm \,m}}    %% meter
%\def\ma         {{\rm \,m}^2}  %% meter squared
%\def\cm         {{\rm \,cm}}   %% centimeter
%\def\cma        {{\rm \,cm}^2} %% centimeter squared
\def\cms         {{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {{\rm \,mm}}   %% millimeter
%\def\mma        {{\rm \,mm}^2} %% millimeter squared
%\def\mum        {{\,\mu\rm m}} %% mu meter
%\def\muma       {{\,\mu\rm m^2}}
%
\def\nm         {{\rm \,nm}\xspace}   %% nanometer
\def\nb         {{\rm \,nb}\xspace}
%%%%%
% Time
%%\def\s{{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {{{\rm \,ps}}\xspace}  %% picosecond
%
% Data processing
\def\kbytes     {{{\rm \,kbytes}}\xspace}
\def\kbsps      {{{\rm \,kbytes/s}}\xspace}
\def\kbits      {{{\rm \,kbits}}\xspace}
\def\kbsps      {{{\rm \,kbits/s}}\xspace}
\def\mbsps      {{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {{{\rm \,Mbytes}}\xspace}
\def\mbps       {{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {{{\rm \,Gbytes}}\xspace}
\def\gbsps      {{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {{{\rm \,Tbytes}}\xspace}
\def\tbpy       {{{\rm \,Tbytes/yr}}\xspace}
%

\def\mic  {{\,\mu{\rm C}}\xspace}
\def\krad {{\rm \,krad}\xspace}
\def\cmc  {{{\rm \,cm}^3}\xspace}
\def\yr   {{\rm \,yr}\xspace}
\def\hr   {{\rm \,hr}\xspace}
\def\degc {{^\circ}{C}\xspace}
\def\degk { {\rm K}\xspace}
\def\degrees{{^{\circ}}\xspace}
\def\mrad{{\rm \,mr}\xspace}               %% milliradian
\def\mradhyph{{\rm -mr}\xspace}
%
\def\sx    {{\sigma_x}\xspace}    
\def\sy    {{\sigma_y}\xspace}   
\def\sz    {{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{{\cal O}}\xspace}
\def\L{{{\cal L}}\xspace}
\def\calL{{{\cal L}}\xspace}
%\def\S{{{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{{\cal S}}\xspace}
\def\calA{{{\cal A}}\xspace}
\def\calD{{{\cal D}}\xspace}
\def\calR{{{\cal R}}\xspace}
\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}
\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\qsq                {{q^2}\xspace}
\def\CP                 {{C\!P}\xspace}
%% Arrows:
\def\ra                 {{\rightarrow}\xspace}
\def\to                 {{\rightarrow}\xspace}
\def\epstag  {{\epsilon_{\rm tag}}\xspace}
\def\tagfac  {{\epstag(1-2w)^2}\xspace}
\newcommand{\stat}{{\mathrm{(stat)}}}
\newcommand{\syst}{{\mathrm{(syst)}}}

% Common combinations
\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {{\sigma_x}\xspace}     
\def\sy    {{\sigma_y}\xspace}   
\def\sz    {{\sigma_z}\xspace}

\def\pbcm {{p^*_{B^0}}\xspace}
%\def\chic1{{\chi_{c1}}}
%\def\chic2{{\chi_{c2}}}
%\def\chic3{{\chi_{c3}}}
\def\chic#1{{\chi_{c#1}}\xspace} % dbm

\newcommand{\etapr}{{\eta^{\prime}}\xspace}
\newcommand{\Betaprks}{{\bz\ra\etapr\KS}\xspace}
\newcommand{\Betaprkz}{{\bz\ra\etapr K^0}\xspace}
\newcommand{\etaprepp}{{\etapr\ra\eta\pipi}\xspace}
\newcommand{\etaprrg}{{\etapr\ra\rho^0\gamma}\xspace}

\newcommand{\inverse}{{^{-1}}\xspace}
\newcommand{\dedx}{{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{{\chi^2}\xspace}
\newcommand{\delm}{{m_{\dstr}-m_{\dz}}\xspace}

\newcommand{\dstr}{{D^{*}}\xspace}
\newcommand{\dstrstr}{{D^{**}}\xspace}
\newcommand{\dsp}{{D^{*+}}\xspace}
\newcommand{\dsm}{{D^{*-}}\xspace}
\newcommand{\dsz}{{D^{*0}}\xspace}
 
\newcommand{\lum} {{\mathcal{L}}\xspace}

% QCD parameters

\newcommand{\as}{{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  {\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  {\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{{A_{\scriptscriptstyle FB}^{#1}}}}
\newcommand{\gv}[1]{{{g_{\scriptscriptstyle V}^{#1}}}}
\newcommand{\ga}[1]{{{g_{\scriptscriptstyle A}^{#1}}}}
\newcommand{\gvb}[1]{{{\overline{g}_{\scriptscriptstyle V}^{#1}}}}
\newcommand{\gab}[1]{{{\overline{g}_{\scriptscriptstyle A}^{#1}}}}


\def\rhobar {{\overline \rho}\xspace}
\def\etabar {{\overline \eta}\xspace}
%\def\paramest {{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {{|V_{ud}|}\xspace}
\def\Vcd  {{|V_{cd}|}\xspace}
\def\Vtd  {{|V_{td}|}\xspace}
\def\Vus  {{|V_{us}|}\xspace}
\def\Vcs  {{|V_{cs}|}\xspace}
\def\Vts  {{|V_{ts}|}\xspace}
\def\Vub  {{|V_{ub}|}\xspace}
\def\Vcb  {{|V_{cb}|}\xspace}
\def\Vtb  {{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{{\sin\! 2 \alpha  }\xspace}
\def\stwob{{\sin\! 2 \beta   }\xspace}
\def\stwog{{\sin\! 2 \gamma  }\xspace}
\def\mistag{{w}\xspace}
\def\dilution{{\cal D}\xspace}
\def\deltaz{{{\rm \Delta}z}\xspace}
\def\deltat{{{\rm \Delta}t}\xspace}
\def\deltamd{{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{{f_D}}\xspace
\newcommand{\fds}{{f_{D_s}}\xspace}
\newcommand{\fsubb}{{f_B}\xspace}
\newcommand{\fbd}{{f_{B_d}}\xspace}
\newcommand{\fbs}{{f_{B_s}}\xspace}
\newcommand{\bsubb}{{B_B}\xspace}
\newcommand{\bbd}{{B_{B_d}}\xspace}
\newcommand{\bbs}{{B_{B_s}}\xspace}
\newcommand{\rgbb}{{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{{\hat{B}_K}\xspace}
\newcommand{\lqcd}{{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}






% Journal References
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\nim}       [1]  {{Nucl.\ Instr.\ and Methods~{\bf #1}}}
\newcommand{\nima}      [1]  {{Nucl.\ Instr.\ Methods {\bf A{\bf #1}}}}
\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}
\newcommand{\jpl}        [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\prep}      [1]  {{Phys.\ Rep.{\bf #1}}}
\newcommand{\jprl}       [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\jpra}       [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jprd}       [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jpre}       [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Th.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}       [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}
\newcommand{\cpc}   [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\mpl}     [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}
\newcommand{\fp}       [1]   {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}  [1]   {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}   [1]    {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\app}  [1]    {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\fizika}[1]   {{Fizika~{\bf #1}}}
\newcommand{\spd}  [1]    {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\baps} [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\araa} [1]   {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\japj} [1]     {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\annp}  [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\ppnp}  [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\prsl}  [1]    {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\apas}  [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\anp}  [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\pan}  [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\cmp} [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\npaps} [1]  {{Nucl.\ Phys.\ A (Proc.\ Suppl.)~{\bf #1}}}

%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}}
\def\bbsim      {\mbox{\tt BBsim}}
\def\beast      {\mbox{\tt Beast}}
\def\beget      {\mbox{\tt Beget}}
\def\Bta        {\mbox{\tt Beta}}
\def\betakfit   {\mbox{\tt BetaKfit}}
\def\cornelius  {\mbox{\tt Cornelius}}
\def\evtgen     {\mbox{\tt EvtGen}}
\def\euclid     {\mbox{\tt Euclid}}
\def\fitver     {\mbox{\tt FitVer}}
\def\fluka      {\mbox{\tt Fluka}}
\def\fortran    {\mbox{\tt Fortran}}
\def\gcalor     {\mbox{\tt GCalor}}
\def\geant      {\mbox{\tt GEANT}}%
\def\gheisha    {\mbox{\tt Gheisha}}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
%\def\jetset    {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}}
\def\minuit     {\mbox{\tt Minuit}}
\def\objegs     {\mbox{\tt Objegs}}
\def\turtle     {\mbox{\tt Decay~Turtle}}
\def\hemicosm   {\mbox{\tt HemiCosm}}
\def\stdhep     {\mbox{\tt StdHep}}
\def\hepevt     {\mbox{\tt{/HepEvt/}}}
\def\squaw      {\mbox{\tt Squaw}}
\def\trackerr   {\mbox{\tt TrackErr}}

